Saliency Driven Image Manipulation

Have you ever taken a picture only to find out that an unimportant background object ended up being overly salient? Or one of those team sports photos where your favorite player blends with the rest? Wouldn't it be nice if you could tweak these pictures just a little bit so that the distractor would be attenuated and your favorite player will stand-out among her peers? Manipulating images in order to control the saliency of objects is the goal of this paper. We propose an approach that considers the internal color and saliency properties of the image. It changes the saliency map via an optimization framework that relies on patch-based manipulation using only patches from within the same image to achieve realistic looking results. Applications include object enhancement, distractors attenuation and background decluttering. Comparing our method to previous ones shows significant improvement, both in the achieved saliency manipulation and in the realistic appearance of the resulting images.

==> fig_attention_shift.tex <==
\begin{figure*}[ht]
		\centering
		\rotatebox{90}{\hspace{0.1cm}}~
		\vspace{0.1cm}
    \begin{subfigure}[b]{.16\textwidth}\includegraphics[width=\textwidth]{multi_8a.jpg}\end{subfigure}~
		\begin{subfigure}[b]{.16\textwidth}\includegraphics[width=\textwidth]{multi_8b.png}\end{subfigure}~
    \begin{subfigure}[b]{.16\textwidth}\includegraphics[width=\textwidth]{multi_8e.jpg}\end{subfigure}~
    \begin{subfigure}[b]{.16\textwidth}\includegraphics[width=\textwidth]{multi_8f.png}\end{subfigure}~
    \begin{subfigure}[b]{.16\textwidth}\includegraphics[width=\textwidth]{multi_8c.jpg}\end{subfigure}~
    \begin{subfigure}[b]{.16\textwidth}\includegraphics[width=\textwidth]{multi_8d.png}\end{subfigure}
		\rotatebox{90}{\hspace{0.1cm}}~
		\vspace{0.1cm}
    \begin{subfigure}[b]{.16\textwidth}\includegraphics[width=\textwidth]{multi_small3a.jpg}\caption{input image}\end{subfigure}~
	  \begin{subfigure}[b]{.16\textwidth}\includegraphics[width=\textwidth]{multi_small3b.png}\caption{input saliency}\end{subfigure}~
    \begin{subfigure}[b]{.16\textwidth}\includegraphics[width=\textwidth]{multi_small3e.jpg}\caption{ours}\end{subfigure}~
    \begin{subfigure}[b]{.16\textwidth}\includegraphics[width=\textwidth]{multi_small3f.png}\caption{ours saliency}\end{subfigure}~
    \begin{subfigure}[b]{.16\textwidth}\includegraphics[width=\textwidth]{multi_small3c.jpg}\caption{OHA}\end{subfigure}~
    \begin{subfigure}[b]{.16\textwidth}\includegraphics[width=\textwidth]{multi_small3d.png}\caption{OHA salinecy}\end{subfigure}
		\caption{\textbf{Saliency Shift.} In these examples the user selected to make salient objects that were not salient in the input images: the lady on the right in the top row and one of the trees in the bottom row. Generating such a saliency shift requires both increasing the saliency of the selected objects and decreasing the saliency of other regions. Our framework succeeds in doing that, as is evident from the saliency maps in (d) that show the woman and the tree are highly dominant. On the contrary, OHA does not provide such a manipulation option, therefore, for example, both trees remain salient in the bottom row. In both examples $\Delta S = 0.6$.}
		\label{fig:attention-shift}
\end{figure*}

==> fig_limitations.tex <==
\begin{figure}[htb]
\captionsetup[subfigure]{labelformat=empty}
		\centering
		\rotatebox{90}{\hspace{0.1cm}}~
		\vspace{-0.2cm}
		 \begin{subfigure}[b]{.19\textwidth}\includegraphics[width=.98\linewidth]{fail_1a_c.jpg}\caption{Input image}\end{subfigure}~
		 \begin{subfigure}[b]{.19\textwidth}\includegraphics[width=.98\linewidth]{fail_1c_c.jpg}\caption{Manipulated Image}\end{subfigure}~
% 		\rotatebox{90}{\hspace{0.1cm}}~
% 		\vspace{0.1cm}
% 		 \begin{subfigure}[b]{.23\textwidth}\includegraphics[width=.98\linewidth]{fail/1c.jpg}\caption{Manipulated Image}\end{subfigure}~
% 		 \begin{subfigure}[b]{.23\textwidth}\includegraphics[width=.98\linewidth]{fail/1d.png}\caption{Manipulated saliency map}\end{subfigure}
		\caption{\textbf{Limitations.} When the input image color set is narrow, the manipulation is limited, making it difficult to enhance a region.}% In this example the user wanted to enhance the gecko but since the image is almost entirely green this did not succeed with our example based approach.}
		\label{fig:limitations}
\end{figure}

